High-Performance and Flexible Parallel Algorithms for Semisort and Related Problems

Semisort is a fundamental algorithmic primitive widely used in the design and analysis of efficient parallel algorithms. It takes input as an array of records and a function extracting a \emph{key} per record, and reorders them so that records with equal keys are contiguous. Since many applications only require collecting equal values, but not fully sorting the input, semisort is broadly applicable, e.g., in string algorithms, graph analytics, and geometry processing, among many other domains. However, despite dozens of recent papers that use semisort in their theoretical analysis and the existence of an asymptotically optimal parallel semisort algorithm, most implementations of these parallel algorithms choose to implement semisort by using comparison or integer sorting in practice, due to potential performance issues in existing semisort implementations. In this paper, we revisit the semisort problem, with the goal of achieving a high-performance parallel semisort implementation with a flexible interface. Our approach can easily extend to two related problems, \emph{histogram} and \emph{collect-reduce}. Our algorithms achieve strong speedups in practice, and importantly, outperform state-of-the-art parallel sorting and semisorting methods for almost all settings we tested, with varying input sizes, distribution, and key types. We also test two important applications with real-world data, and show that our algorithms improve the performance over existing approaches. We believe that many other parallel algorithm implementations can be accelerated using our results.

==> algo-semisort.tex <==
\begin{algorithm}[t]
    \small
    \caption{The semisort algorithm\label{alg:semisort}}
    \KwIn{The input array $A$, a hash function $h$, and a comparison function $\comp$}
    \KwOut{The semisort result $A$ (inplace)}
    \SetKwInOut{Maintains}{Maintains}
    \SetKwProg{myfunc}{Function}{}{}
    \SetKwFor{parForEach}{ParallelForEach}{}{endfor}
    \Maintains{\xiaojun{This is the parameter space, not maintains.} \\
        $\alpha$: base case size \\
        $\sigma$: sample multiplier \laxman{We used $\beta$ for the block size earlier}\yihan{I changed it to $\sigma$}\\
        $n_L$: the number of light buckets \\
    }
    \lIf {$|A| < \alpha$} {
        \Return{Semisort $A$ sequentially} \DontPrintSemicolon \label{line::basecase}
    }
    $S \gets$ Sample $\sigma\log n$ keys \label{line:sample}\yihan{But is this value $\sigma$ important? Can we just say sample ``$O(\log n)$'' keys?}\\
    Count the occurrences of each key in $S$ \label{line:count}\\
    Initialize the heavy table $H$ \\
    \For {each distinct key $k \in S$ } {
        \If {the occurrences of $k$ is at least $\log n$} {
            Insert $k$ into $H$ \label{line:insert}\\
        }
    }
    $n_H \gets$ number of distinct keys in $H$ \\
    $\offsets \gets$ parallel count sort $A$ with $\mf{GetBucketId}$ \label{line:count_sort}
    \parForEach {$i \gets 1, \cdots, n_L$} {
        \mf{Semisort}$(A.\text{subarray}(\offsets[i], \offsets[i+1]), h, comp)$ \label{line:recursion}
    }

    \myfunc{\upshape \mf{GetBucketId}$(k, H, h, n_L)$} { \label{line:bucketid}
        \lIf {$k$ is found in $H$} {
            \Return{the heavy id of $k$ in $H$} \DontPrintSemicolon
        } \lElse {
            \Return{$n_H + (h(k) \mod n_L)$} \DontPrintSemicolon
        }
    }

    \end{algorithm}


==> algo.tex <==
\section{Our Semisort Framework (\SMS{})}

In this section, we present our algorithm for \semisort{} and related problems.
All of our algorithms are designed on top of our proposed \Semisort{} Framework (\SMS{} framework). In the following, we first present the framework, and then describe the algorithms in detail.
\begin{table}
  \centering
  \begin{tabular}{ll}
    \hline
    % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
    \multicolumn{2}{@{}l}{\textbf{Input:}}\\
    $A$ & input array of \record{s} in universe $U$ \\
    $K$ & key type of \record{s}\\
    $k(\cdot)$ & $k:U\mapsto K$ extracts the key of a \record{} \\
    $=_K$ & (or $=$) equality test on keys \\
    $<_K$ & (or $<$) less-than test on keys \\
    $h(\cdot)$ & \userhash{}; $h:K\mapsto [0, n^{\hashrange}]$\\
    $\combine$ & combine operation for \collectreduce{}\\
    \multicolumn{2}{@{}l}{\textbf{Parameters:}}\\
    $\threshold$& desired number of heavy/light \bucket{s}\\
    $\B$ & \block{} size\\
    $p$ & sample rate\\
    \multicolumn{2}{@{}l}{\textbf{Used in the algorithm:}}\\
    $\nlight$& number of light \bucket{s}\\
    $\nheavy$& number of heavy \bucket{s}\\
    $\heavyhash$ & \heavytable{}; Maps heavy keys to \bucket{} ids\\
    $B$ & output of \semisort{}\\
    $\countm$ & \countmatrix{}\\
    $P$ & prefix sum of $\countm^\matrixtrans$ (row-major)\\
    \hline
  \end{tabular}
  \vspace{.01in}
  \caption{Notation and parameters used in our framework.}\label{tab:notation}
\end{table}

\begin{algorithm}
\caption{The Semisort Framework (\SMS{})}\label{algo:framework}
%\KwIn{An array $A$ of \record{s}, a function $k(\cdot)$ to extract the key of a \record{}, a \userhash{} function $h$, an equality test function $=$ and a less-than test function $<$, and possibly an associative binary combine operation $\combine$ (only for \collectreduce{}).}
%\KwOut{An array $B$ with all \record{s} in $A$ and all identical keys contiguous with each other (for \semisort{}), or a mapping from each distinct key to the sum of \record{s} (w.r.t. $\combine$).}

\textbf{\sampling{}.} Sample and determine the heavy keys. 
Heavy keys use an individual bucket; multiple light keys share a \bucket{}.\\

\textbf{\counting{}.} Split the input into \block{s} and process each \block{} in parallel. Within each \block{}, count the \record{s} falling into each \bucket{}. \\

\textbf{\placing{}.} Assign appropriate memory for each \bucket{}, Then in parallel, process each \block{} to place each element into its corresponding \bucket{}.\\

\textbf{\refining{}.} Locally \semisort{} the light \bucket{s} to gather identical keys in the same \bucket{}.

\end{algorithm}
\subsection{\Semisort{} Framework and algorithm}

\myparagraph{\sampling{}.} Similar to \BGSS{} algorithm, the first step of our \SMS{} framework is also to take a set $S$ of samples, in order to distinguish heavy and light keys. 
Let $p$ be the sample rate, which means that each \record{} is sampled with probability of $p$.
Similar to \BGSS{} algorithm, we will let each heavy key take an individual bucket, and let multiple light keys share a \bucket{}.
The \emph{heavy keys} are identified as keys appearing many times in the sample, such that we would expect their actual number of occurrences to be large with higher confidence.
Using standard concentration inequalities, a heavy key must appear $\Omega(\log n)$ times in the samples to enable an accurate estimation.
We use $\nheavy$ to denote the actual number of heavy buckets.
The \emph{light keys} are grouped into $\nlight$ light \bucket{s} by evenly partitioning the hash range into $\nlight$ subranges.
To ensure the desired bound \laxman{what is the desired bound?}, we want the number of heavy \bucket{s} to be approximately the same as the number of light \bucket{s}, and thus we use a tunable parameter $\threshold$ to control the (approximate) number of heavy or light buckets used in the algorithm (i.e., $\threshold\approx \nlight \approx \nheavy$).
\laxman{How about putting some of the terms defined here in \\defn\{\}? Should the definition of $\threshold$ in the table include ``approximate''?}
For the number of light \bucket{s}, we can simply set $\nlight=\threshold$. 
For heavy \bucket{s}, if we identify all keys with $\Omega(\log n)$ samples as heavy key, this indicates that the sample rate $p=\Omega(\threshold\log n/n)$.\laxman{end of last sentence is confusing---this indicates that we should set our sample rate to $p = \ldots$?}
In total, we will maintain $\nlight + \nheavy$ buckets, the first $\nlight$ buckets are light \bucket{s} and the other $\nheavy$ \bucket{s} are heavy \bucket{s}.
\laxman{Is previous sentence adding anything important?}
After the heavy keys are identified, they are placed in the hash table $\heavyhash{}$ associated with their \bucket{} labels, referred to as the \emph{\heavytable}, so that later steps can look up if a key is heavy or not.

\myparagraph{\counting{}.} The goal of this step is to count the \emph{exact} number of elements in each \bucket{}.
To make this step parallel and I/O-efficient, the input sequence will be evenly divided into \block{s} of size $\B$.
We than process each of the \block{s} in parallel. We count the number of elements in each bucket in a $(\nlight+\nheavy)\times (n/\B)$ matrix $\countm$, referred to as \emph{\countmatrix}.
In particular, $\countm_{ij}$ is the number of \record{s} in \block{} $i$ falling into \bucket{} $j$.
In more detail, within each \block{} $i$, the algorithm determines which bucket each key $k$ belongs to.
The algorithm first looks up the \heavytable{} $\heavyhash$ to determine if $k$ is a heavy key, and if so, it obtains the bucket label $j$ from $\heavyhash$.
\laxman{Using bucket label and bucket ids interchangeably. How about id, as it's shorter?}
Otherwise, since the light buckets are determined by evenly partitioning the hash range of \userhash{} function $h$, the light bucket id is simply $j=\lfloor h(k)/\B \rfloor$. It then adds one to the corresponding cell in $\countm_{ij}$.

\myparagraph{\placing{}.} We will now place each \record{} to an appropriate position in the output (for \semisort{}), or gather all relevant \record{s} together (for \collectreduce{} and \histogram{}). 
%In the following, we use \semisort{} as an example to explain our \SMS{} framework. 
\laxman{Should formally define \collectreduce{}, \histogram{} in prelims before this part.}
% Later in \cref{sec:collectreduce}, we present
These can all be performed using the information in $\countm$.
For example, the size of each \bucket{} can be computed by taking the sum of each column in $\countm$. 
Therefore, we can directly allocate exactly the necessary space per bucket. 
Specifically, we allocate space for all of the \bucket{s} as a contiguous chunk of memory, referred to as an array $B$, and the \bucket{s} are only (conceptually) separated by using offsets in $B$.
%
%
In fact, we will also take the prefix sum over the entire matrix $\countm$ in column-major to obtain the matrix $P$. 
\laxman{``we will also'' $\rightarrow$ ``we take''? This is the only sum we take, right? This last sentence is confusing since $P$ is in row-major order, but it sounds like it could be column-major.}
When we process a \record{} in \block{} $j$, if a \record{} falls into \bucket{} $i$, it should be written to $B$ starting from position $P_{ij}$.
In order to compute this prefix sum I/O-efficiently, we will first compute the transpose of the \countmatrix{} $\countm^\matrixtrans$ and then compute the prefix sum in row-major in matrix $P$.

Note that for \collectreduce{} or \histogram{}, it is unnecessary to distribute the heavy keys to their corresponding \bucket{}. %What matters is the \abstractsum{} of each key. 

\myparagraph{\refining{}.} 

\laxman{We have presented GSSB in Section 3, and there is a decent amount of overlap between that description and our description here. I believe an unfamiliar reader will be confused as to what is new here. Shall we try to very explicitly comment on this in a sub-section on \emph{what is new in our framework} from GSSB? Things we have discussed include: 
\begin{itemize}
\item multiple levels allows us to identify more heavy keys; heavy keys are good for the algorithm
\item no assumption that the inputs are hashed keys; our framework is more general and supports arbitrary records and keys equipped with lt or eq,
\item (related to generality) supporting both \semieq{} and \semile{},
\item (related to generality) supporting generalizations of semisort (histogram, collect-reduce), 
\item significantly lower space usage,
\item better cache-performance (could quantify this experimentally by measuring L3 misses, if time). 
\end{itemize}
I guess some of these points are experimental, but if we clarify how these points became possible due to the framework/algorithm design, they would fit in this discussion. Another place we could have this discussion is after Section 5.}


==> imp.tex <==
\section{Implementation Details}

We note that although our algorithms are conceptually simple and similar to
some existing algorithms in some steps, our selection of parameters and careful
application of I/O-efficient optimization techniques also contributes to the
practicality of our algorithms. We briefly present an important optimization in
this section.

\myparagraph{In-place/out-of-place Switching.}
The performance of sorting algorithms can suffer due to excessive data movement.
This is the reason why most in-place algorithms can naturally achieve fewer
cache-misses, and thus relatively good performance.
%
If the output elements are written to the input array, we refer to as
\defn{in-place}. Otherwise, if they are written to a new array, we refer to as
\defn{out-of-place}.
%
To implement sorting algorithms in-place, a temporary array is needed by our
algorithms such that in the \counting{} step, the elements can be placed into
this array without affecting the elements in the input array.
%
Finally, a copy step is followed to move the elements from the temporary array
to the output array.
%
To minimize data movement, for light buckets, we use the temporary array as the
input, and perform an out-of-place sort in the next level of recursion.
%
This optimization can keep the algorithms from moving the elements back and
forth in the temporary array and the output array and save an extra round of
copies.
%
We note that this technique only works for semisort and does not work for
collect-reduce and histogram, as the input/output types may not be the same in
these two applications.


==> problem.tex <==
\section{Problem Definition}

In this section, we formally define \semisort{} and relative problems.

\paragraph{\Semisort{}}
As mentioned, 

==> response/eliminating_writes.tex <==
%\subsection*{Common Concern 3: Benefits of eliminating writes}
This section is to address \textbf{W1 and D1 of Reviewer 3}.
\answer{Revision is in Section 5.1.} We include our response to this
question in the common section since we feel our response touches upon
concerns that are

%W1. The reasons and the benefits of eliminating writes need to be
%further discussed and evaluated.
%D1.The authors claim several benefits of the setting of eliminating
%writes in the introduction. However, it is still unclear whether
%eliminating writes will definitely perform better than the algorithms
%that contain a small percentage of writes. Empirical studies or
%discussions are expected to show this point if the theoretical proof
%cannot be provided.


==> response/intro.tex <==

We would like to thank all of the reviewers for their helpful
critiques, feedback, and questions. The revised version of this paper
represents a substantial effort on our part to address the reviewers'
critiques as well as improve the presentation of our paper based on
the reviewers' feedback. \revised{We have highlighted new changes in
our paper for this revision in a forest-green color.}
%
We list the major changes in the revised paper as follows:
\begin{itemize}[topsep=1pt,itemsep=0.2pt,parsep=0pt,leftmargin=15pt]
  \item {\bf Section 3 (Parallel Semi-Asymmetric Model)}: We made a
  number of changes to improve the model section:

  \begin{itemize}[topsep=1pt,itemsep=0.2pt,parsep=0pt]
    \item We thoroughly rewrote the section on external-memory models
    to make it clear what the main differences are between the PSAM
    and other 2-level memory models.

    \item We included a figure depicting the model, making it clear
    that there are two variants of the model (a regular and relaxed
    model), and that the asymmetry of writes to the \largemem{} is a
    major feature of our model.

    \item We added a section on the applicability of the \SAMabbrev{},
    discussing both other problems that our model could be applied to,
    as well as pointing out instances where certain problems seem to
    require performing writes in our model.

  \end{itemize}


  \item {\bf Section 4 (Sage)} We significantly rewrote and reorganized
  this section in response to the reviewers' feedback:
  \begin{itemize}

    \item We reordered this section to first introduce
    the building-blocks and primitives used to obtain efficient
    algorithms in Sage, before diving into the theoretical bounds our
    algorithms have in the \SAMabbrev{}. The original submission
    inverted this order, introducing our graph algorithms and their
    bounds before introducing the primitives, which was potentially
    confusing.

    \item Based on the reviewer's suggestions, we updated Table 1 to
    include a comparison of the bounds obtained by converting existing
    GBBS algorithms to run on NVRAMs in the \SAMabbrev{} vs. the
    efficient bounds \oursystem{} algorithms obtain in the
    \SAMabbrev{}.

    \item Based on the reviewer's suggestions, we included an
    end-to-end case study of how to implement a ubiquitous
    breadth-first search (undirected shortest-paths) algorithm using the
    provably-efficient primitives Sage. For this problem, which shares
    many similarities with other algorithms we design in this paper,
    we provide work-depth analysis in the \SAMabbrev{}.

    \item We re-organized the algorithms section to better explain how
    the theoretical bounds obtained in Table 1 can be derived using
    the theorems proved about the filtering primitive and traversal
    primitive (designed in this paper). We emphasize that the complete
    proofs and algorithm details rely on our previous
    work~\cite{dhulipala18scalable}. We hope the reviewers understand
    that it is impossible due to space constraints for us to provide completely self-contained
    descriptions and algorithms for all 18 problems in this paper, and
    hope that illustrating how the proof is done in full detail for
    one problem (BFS), and providing clear descriptions of how the
    other results are obtained using the new theorems for filtering
    and traversal from this paper combined with the results from our
    previous work is helpful. We will provide full
    problem-specifications and algorithm descriptions in the full
    version of this paper, which we would be happy to provide to the
    reviewers~\cite{dhulipala2019semi}.

  \end{itemize}

  \item {\bf Section 5 (Experiments)}. We made several changes to
    this section to improve readability and make our conclusions clearer.
    \begin{itemize}[topsep=1pt,itemsep=0.2pt,parsep=0pt]
      \item We added a summary of our main experimental results at the
      start of this section as suggested by Reviewer 3.

      \item We updated Figure 5 to make it clear that we are plotting
      the \emph{speedup} of each algorithm on the y-axis, and
      now explicitly state in the figure that we show the parallel
      running time of each experiment on top of the bar.

%      \item We include additional details about the benefits of
%      completely eliminating writes to the \largemem{} in our
%      approach. We also address this point in further detail below.
    \end{itemize}

\end{itemize}

%\noindent We also carefully polished the paper.


==> response/psam_vs_others.tex <==
\subsection*{Common Concern 1: Differences between the \SAMabbrev{}
and other existing models}
This section is to address
{\bf W1} and {\bf D1} of Reviewer 1,
and {\bf W1} of Reviewer 2. \answer{This revision occurs in Section 3.}
%
We thank the reviewers for their helpful comments about this topic. We
acknowledge that the comparison to existing two-level models, and
other models in general was lacking, and rewrote Section 3.3 to
address this issue. We also expanded the ``discussion'' section about
our model to address some of the reviewer concerns, which we consider
below.

\myparagraph{Differences between \SAMabbrev{} and two-level models}
To address Reviewer 1's feedback ({\bf W1}), we revised our discussion
to compare the \SAMabbrev{} with both the \EM{} and \SEM{} models. We
now list what we believe are the three main differences between the
two models, namely the fact that (i) the \SAMabbrev{} accounts for the
cost of reading and writing to the fast-memory (\smallmem{} in our
paper), whereas the \EM{} and \SEM{} models do not, (ii) the
\SAMabbrev{} does not issue I/Os to the external memory (\largemem{}
in our paper) in blocks of size $B$ since NVRAMs are byte-addressible,
and (iii) the \SAMabbrev{} explicitly models the asymmetry of NVRAMs,
which is not captured by either the \EM{} or \SEM{} models, where both
reads and writes to the large memory cost $B$.

\myparagraph{Reasons for proposing the \SAMabbrev{}}
Next, we address Reviewer 2's feedback ({\bf W1}). This follows up on
our response to Reviewer 1. We made changes throughout Section 3 to
make it more clear what the main differences are between the
\SAMabbrev{} and existing related models (such as two-level models,
existing asymmetric models, and the semi-streaming model). To the best
of our knowledge there is no setting of parameters using existing
models that captures the \SAMabbrev{} model.


%Reviewer 1
%W1. The difference between PSAM and the existing two-level models are
%not clearly clarified in Section 3.1.
%D1. The paper is largely based on the PASM model. However, it’s not
%clearly clarified of the difference between PSAM and the existing
%memory models in Section 3.1.
%
%- Similar to the NVRAMs, we can also observe significant difference
%  between the write and read costs on some types of traditional
%  external memory devices such as SSD. Are the memory models for these
%  devices applicable for NVRAMs?
%
%- An essential advantage of NVRAMs is the byte-addressability. But the
%  graph data in Sage is stored in the CSR format on NVRAM, which is
%  organized as blocks regarding to each vertex. If so, there is no
%  difference between the PSAM and the semi-external memory model
%  (Section 3.2). It seems that the block-based design for the
%  semi-asymmetric graph filtering violates the PSAM model.
%
%- In addition to the previous question, we want to know the cost
%  difference between random read and blocked read on NVRAM.


% Reviewer 2
%W1: The comparison with other relevant models shall be discussed in
%details. The discussion in Section 3.2 is very briefly, which can not
%be convincing for audience why the new model shall be proposed. Can
%the primitives for PSAM be captured by any existing models?



==> response/reviewer_1.tex <==
\subsection*{Response to Reviewer 1}
\noindent We have addressed specific parts of the reviewer's helpful
feedback which were shared with the other reviewers in the common
concerns above, specifically items {\bf W1} and {\bf D1} which
concerns the relationship between the \SAMabbrev{} and other two-level
memory models, and {\bf W2}, {\bf W3}, {\bf R1}, and {\bf R2}, which
concern adding examples to illustrate how an algorithm is implemented
in \oursystem{}, and improving the exposition of our work-depth bounds
for our algorithms in Section 4.

We address the remaining comments
below (parts of {\bf D1} and {\bf D3}).

\commentx{D1}{\textbf{}
\answer{This revision occurs in Section 3.}}{
%- Similar to the NVRAMs, we can also observe significant difference
%  between the write and read costs on some types of traditional
%  external memory devices such as SSD. Are the memory models for these
%  devices applicable for NVRAMs?
%
We partly addressed this comment in Common Concern 1
(comparing the \SAMabbrev{} and other existing memory models). We now
address the remaining questions about memory models, and the costs of
primitives.


\myparagraph{Cost of Reads and Writes on External Memory Devices}
We agree with the reviewer that there is some asymmetry in the
cost of reads and writes on existing external memory devices.
However, \emph{both reads and writes} to these devices are at
least one order of magnitude more expensive than reads and writes to
DRAM. Existing models that model these devices, such as the \EM{}
and \SEM{} model, consider the cost difference between reads and writes
to be relatively small, and abstract both reads and writes to the external memory
to the same cost bucket. By contrast, the performance of NVRAM is much closer
to that of DRAM, making the difference between reads and writes more significant.

%- An essential advantage of NVRAMs is the byte-addressability. But the
%  graph data in Sage is stored in the CSR format on NVRAM, which is
%  organized as blocks regarding to each vertex. If so, there is no
%  difference between the PSAM and the semi-external memory model
%  (Section 3.2). It seems that the block-based design for the
%  semi-asymmetric graph filtering violates the PSAM model.
\myparagraph{Block-Based Design in Semi-Asymmetric Filtering}
We have made changes to better explain the difference between the
\SAMabbrev{} and the \EM{} and \SEM{} models in Section 3.3. The
reviewer also mentions that the CSR format on NVRAM is stored
contiguously. We emphasize that although the format stores edges
incident to each vertex contiguously, the data itself is
byte-addressible, and there is no restriction in the hardware forcing
reads to writes to be at the granularity of an entire block (e.g., 4Kb).
This fact is preciscely what makes our
semi-asymmetric graph filter work in the relaxed \SAMabbrev{}
using $O(n + m/\log n)$ words of DRAM, since if a bit corresponding to
some edge is set in DRAM, we can fetch the edge data (using a read to the NVRAM)
at unit cost. We thank the reviewer for encouraging us to explain this more clearly.

\input{table_blocking}

%- In addition to the previous question, we want to know the cost
%  difference between random read and blocked read on NVRAM.
\myparagraph{Cost of Blocked Reads vs. Random Reads}
This is a great question. We ran a simple micro-benchmark to compute
the difference in running time between both random reads and blocked
reads on NVRAMs. The benchmark consists of an array $A$ of $1$ billion
8-byte elements, allocated on a single socket's NVRAM. All threads are
from the same socket. We consider two primitives:
\begin{enumerate}[label=(\textbf{\arabic*}),topsep=1pt,itemsep=0pt,parsep=0pt,leftmargin=15pt]
\item Blocked-Read. The primitive performs a reduction on an array
where the $i$-th element is $A[i]$. The output is $s = A[0] + \ldots +
A[n-1]$.
\item Random-Read. The primitive performs a reduction on a delayed
sequence (a lazy view) of $A$ called $S$. The $i$-th element of $S$ is
computed by generating a random index $r_i \in [0, n)$ and returning
$S[i] = A[r_i]$. The output is $s = S[0] + \ldots + S[n-1]$.
\end{enumerate}
To illustrate the effect of blocking on DRAM, we also ran the
experiment on DRAM to see what the difference between blocked reads
and random reads is in a purely in-memory setting. The results are
shown in Table~\ref{table:blocking}. This experiment shows that
the performance difference between blocked and random reads on
NVRAM is similar to that on DRAM. This reinforces our belief that
blocking is not worth parameterizing in the \SAMabbrev{}.

We observe that there is a significant difference between random and
blocked reads in both the NVRAM and DRAM settings. In NVRAM, the cost
of reading $1$ billion random array locations is 27.4x slower than
reading consecutive array locations, which has excellent locality. On
DRAM the cost is 15.5x slower to read random locations vs. reading
consecutive array locations. Note that the total number of bytes read
is significantly higher for random reads vs. blocked reads, since each
random read is likely to be a cache-miss.

Ultimately, taking into account locality and designing algorithms that
avoid random reads as much as possible is still crucial for
performance whether on DRAM or on NVRAM.
}


\commentx{D3}{\textbf{Graph Algorithm Explanations}
\answer{This revision occurs in Section 4.}}{
We apologize for the lack of detail for the algorithms considered in
this paper, but unfortunately due to the space constraints it was very
difficult to fully review and re-present all of the
algorithmic components from our previous paper in this paper while
presenting our new techniques in the \SAMabbrev{}, as well as a broad
set of experimental results.

We tried to strike a balance that provides enough details so that the
interested reader can read an algorithm description in the full
version of our SPAA paper~\cite{dhulipala18scalable}, and combine this
description with the additional improvements and optimizations made in
the \SAMabbrev{} model to generate an implementation of our
\SAMabbrev{} graph algorithm. To help with this process, based on the
reviewer's recommendation we provided a case-study of a complete
implementation of BFS in \oursystem{}, illustrating both the actual
code and the work-depth analysis in the model. We believe providing
this example will help a reader who is unfamiliar with the
Ligra interface~\cite{ShunB2013} understand how algorithms are implemented in
\oursystem{} and make the system more accessible.
}


==> response/reviewer_2.tex <==
\subsection*{Response to Reviewer 2}
\noindent We have addressed the parts of the reviewer's helpful
feedback that were shared with the other reviewers in the common
concerns sections above, specifically items {\bf W1} and {\bf W2},
which concern our theoretical bounds and the choice of the work-depth
model. We provide our responses to the reviewer for items {\bf W3},
and {\bf D1--D5} below.


\commentx{D1}{\textbf{Filtering Interface Improvement.}
%D1: In Section 4.2.2, the filter interface is defined as four
%primitives. It is not very clear why we want to keep both MakeFilter
%and MakeAsymFilter. The two has the same interfaces, but just
%different type of the input graph. Will it be reasonable to view them
%as two specific cases under the same interface design.
\answer{This revision occurs in Section 4.1.}}{
The correctly identifies that the two constructors in the filtering interface
are differ only in input. Accordingly, we combined the constructors into
a single constructor that takes into account the directionality of the
filter.
}


\commentx{W3 and D2}{\textbf{Algorithm Costs in a Baseline Model.}
\answer{This revision occurs in Section 4.}}{
We thank the reviewer for this helpful suggestion, which led us to
improve Table 1 which displays the work and depth bounds of
\oursystem{}. In addition to our bounds, we now show the work bounds
obtained by applying the GBBS algorithms in the \SAMabbrev{} model.
The bounds for GBBS Work correspond directly to the experiment we
consider in Section 5 that runs GBBS algorithms over NVRAMs using
libvmmalloc to perform memory allocations on the NVRAM. The goal of
this illustration, and of our experiment is to show that having a
better model encourages people to write more efficient algorithms. We
hope that illustrating the theoretically inefficient bounds that are
obtained when algorithm design is not closely coupled with the target
theoretical model helps better motivate our work.
}


\commentx{D3}{\textbf{Data Organization of Graph Filter.}
\answer{This revision occurs in Section 4.1.1.}}{
  Per the reviewer's request, we have rewritten this section to help
  make it clear that our data structure is similar to the CSR
  structure rather than identical to it, and to emphasize the difference.
  The major conceptual difference is that the blocks in the filtering
  structure correspond to subsets of the edges in the CSR structure.
  As edges are deleted, the blocks become empty
  and are then compacted out of the graph filter structure.
}



%D4: In Section 5.5, the analysis may need further attention. It is not
%very clear in the section the speedup is observed from experiment, or
%from the proposed framework. We need such analysis to justify the
%significance of the proposed framework.
%
%D5: Performance profiling shall be conducted for some algorithms to
%show the performance bottlenecks, if any. This seems not effectively
%done in the current paper.

\commentx{D4 and D5}{\textbf{Speedup and Performance Profiling.}
\answer{This revision occurs in Section 5.}}{
\input{table_perf}
We thank the reviewer for this helpful question. To answer the
reviewer's question, we ran our \oursystem{} code on the ClueWeb
graph, which is the largest graph that fits entirely in DRAM. Our goal
was to compare the performance obtained by \oursystem{} in DRAM, and
the performance obtained by \oursystem{} in NVRAM to see whether there
are any bottlenecks that emerge in the NVRAM execution.

Table~\ref{table:perf} displays performance counters including the
{\bf total number of cycles}, {\bf cycles stalled waiting on L3}, {\bf
L2 and L3 Hit Ratios}, and {\bf L2 and L3 Misses} for the experiment
for several graph problems on the ClueWeb graph. We gathered all data
other than the cycles stalled using Open PCM (OPCM), a widely-used
open-source version of Intel's PCM tool, and
gather the stalled cycles data using perf. We double-checked that the
results returned from OPCM match those returned by perf for aggregate
statistics that both report.

First, we observe that the ratio of running times is reliably
predicted by the ratio of total cycles. Second, other than the total
number of cycles stalled waiting for L3, the other statistics are
remarkably similar between the NVRAM and DRAM runs. We expected this,
since the algorithm is implemented identically other than whether the
data is fetched from NVRAM or DRAM. Finally, we observe that the total
number of cycles stalled in L3 (i.e., the cycles stalled waiting on a
pending load is consistently higher for the NVRAM run). Although our
techniques eliminate a large fraction of NVRAM accesses compared to
naive techniques, such as using libvmmalloc, the cycles stalled
statistic reflects the fact that NVRAM accesses have higher latency
than DRAM accesses.
}


==> response/reviewer_3.tex <==
\subsection*{Response to Reviewer 3}
\noindent We thank the reviewer for their very helpful feedback. We
provide our responses to all of their comments below.

\commentx{W1 and D1}{\textbf{Benefits of Eliminating Writes.}
\answer{This revision occurs in Section 3.}}{
Thanks to the reviewer for this helpful comment, which led to us
carefully clarifying our goals in the paper. Specifically, we have
changed the paper to make it clear that our main goal was not to show
that performing no-writes is strictly superior to any solution that
performs some writes, but to show that, perhaps surprisingly, not
performing any writes is consistently effective and outperforms
state-of-the-art existing approaches to programming NVRAM graph
algorithms. Furthermore, the \SAMabbrev{} is well-suited for studying
algorithms that perform a small number of writes, and it is an
interesting question for future work whether such algorithms can
outperform the strict discipline of avoiding writes that was used this paper.
We are interested in studying this question for future work.
}

\commentx{W2 and D2}{\textbf{Discussion of other fundamental problems.}
\answer{This revision occurs in Section 3.2.}}{
Thanks to the reviewer for this helpful question, which helped us
improve our discussion of the model in Section 3. Specifically, we
added a discussion about the applicability of our model. We have added
discussion of other fundamental graph problems, and whether it is
possible to implement them in the \SAMabbrev{} model. For problems
such as clique-search, a local-search variant of SimRank, and local
clustering problems such as personalized PageRank, we
believe that existing approaches can naturally be adapted to the
\SAMabbrev{} model, since these algorithms all use only $O(n)$ words
of memory.

However, some problems, such as $k$-Truss, $(r,s)$-nucleus
decomposition, and possibly subgraph matching and frequent subgraph
mining may require significantly more than $O(n)$ space to store the
output of the algorithm. In these cases, we believe that the
\SAMabbrev{} model may still be a useful guide for algorithm design,
since although a number of writes may be unavoidable, designing
algorithms to minimize the number of writes, or minimize the number of
bytes written is still likely to lead to more efficient algorithms. We
note that in ongoing work we are currently studying memory-efficient
compression techniques for solving $k$-Truss on massive graphs, and
plan to experimentally evaluate our work in the NVRAM setting by
working in the \SAMabbrev{} setting and performing writes to store and
update the trussness values.
}

\commentx{D3}{\textbf{Speedup of our Algorithms.}
\answer{This revision occurs in Section 5, Figure 6.}}{
We sincerely apologize for this confusion. Our figure in the previous
submission did not make it clear that the height of the bar depicts the
speedup, and that the values on top of the bars are the actual
parallel running times of the codes. We have made a significant effort
to improve the figure, which now explicitly states that the values on
top of the bars are parallel (96-thread) running times both in the figure
itself and in the caption.
}

\commentx{D4}{\textbf{Summary Paragraph in Experiments.}
\answer{This revision occurs in Section 5.}}{
We appreciate this useful suggestion! We added a list of our main
results to the beginning of the experimental section,
along with pointers to the relevant sections, and hope that the
section is more clear because of this change.
}

\commentx{W3 and D5}{\textbf{Presentation.}
\answer{This revision occurs throughout the paper.}}{
Thanks for this helpful comment. We made several careful passes over
the entire paper to fix our language usage and improve the overall
quality of our presentation.
\begin{itemize}[topsep=1pt,itemsep=0.2pt,parsep=0pt,leftmargin=15pt]
  \item We completely reorganized the presentation of Section 4.
  Previously, we started off by discussing our graph algorithm
  results (which rely on  and graph filtering)
  \emph{before} discussing these semi-asymmetric techniques. The new
  order first provides an overview of the section, introduces our
  techniques, provides a case-study of a \SAMabbrev{} algorithm, and
  lastly describes our graph algorithmic results. We hope that this
  significant reorganization makes the paper more clear.

  \item We added more figures, both for the model, and to provide the
  actual \oursystem{} code for BFS as part of a case-study.

  \item Lastly, we made a significant effort to fix typos and improve
  the clarity of our writing.
\end{itemize}
~
}


==> response/table_blocking.tex <==
\begin{table}[!t]\footnotesize
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabular}[!t]{l|r@{  }|r@{  }}
\multicolumn{1}{c|}{Configuration} & \multicolumn{1}{c|}{Experiment} & \multicolumn{1}{c}{Running Time}\\
\midrule
NVRAM    & Blocked-Read     & 0.255 \\
NVRAM    & Random-Read      & 6.99  \\
DRAM     & Blocked-Read     & 0.102 \\
DRAM     & Random-Read      & 1.59  \\
\end{tabular}
\captionof{table}{\label{table:graphinfo}\small Performance differences between
blocked reads and random reads on both NVRAM and DRAM.}
\label{table:blocking}
\end{table}
%DRAM,reduce,0.102
%DRAM,reduce-gather,1.59
%NVRAM,reduce,0.255
%NVRAM,reduce-gather,6.99


==> response/table_pref.tex <==
\begin{table}[!t]\footnotesize
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabular}[!t]{l|l@{  }|c|c|c|c|c|c|c}
\multicolumn{1}{c|}{Configuration} & \multicolumn{1}{c|}{Algorithm} &
\multicolumn{1}{c}{Running Time} &
\multicolumn{1}{c}{Total Cycles} &
\multicolumn{1}{c}{Cycles Stalled in L3} &
\multicolumn{1}{c}{L2 Hit Ratio} &
\multicolumn{1}{c}{L3 Hit Ratio} &
\multicolumn{1}{c}{L2 Misses} &
\multicolumn{1}{c}{L3 Misses}\\
\midrule
NVRAM    & BFS & 2.45 & 816B & 201B & 0.168 & 0.187 & 705M & 304M \\
DRAM     & BFS & 2.09 & 659B & 127B & 0.172 & 0.189 & 690M & 294M \\
\midrule
NVRAM    & Connectivity & 8.31 & 2.55T & 399B & 0.165 & 0.121 & 2.00B & 1.25B \\
DRAM     & Connectivity & 7.95 & 2.40T & 329B & 0.165 & 0.118 & 2.00B & 1.27B \\
\midrule
NVRAM    & MIS & 12.9 & 3.45T & 873B  & 0.199 & 0.099  & 3.46B & 2.39B  \\
DRAM     & MIS & 12.0 & 3.29T & 639B  & 0.201 & 0.103  & 3.38B & 2.30B \\
\midrule
NVRAM    & $k$-Core & 70.3 & 18.8T & 5.12T & 0.242 & 0.098 & 19.0B & 12.8B \\
DRAM     & $k$-Core & 66.0 & 17.8T & 4.79T & 0.237 & 0.097 & 20.2B & 13.6B \\
\end{tabular}
\captionof{table}{\small Performance differences between
blocked reads and random reads on both NVRAM and DRAM.}
\label{table:perf}
\end{table}


% 159,441,203,506 (noop)
% 155,335,854,876 (noop)


==> response/table_times.tex <==
%\setlength{\tabcolsep}{2pt}
\begin{table}[!t]\footnotesize
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabular}[!t]{l|r@{  }|r@{  }|c}
\multicolumn{1}{c|}{Graph Dataset} & \multicolumn{1}{c|}{Num. Vertices} & \multicolumn{1}{c|}{Num. Edges} & $\davg$\\
\midrule
{\emph{LiveJournal}~\cite{boldi2004webgraph} }       & 4,847,571        &85,702,474        &  17.6 \\
{\emph{com-Orkut}~\cite{Yang2015}  }                 & 3,072,627        &234,370,166       &  76.2 \\
{\emph{Twitter}~\cite{kwak2010twitter}  }            & 41,652,231       &2,405,026,092     &  57.7 \\
{\emph{ClueWeb}~\cite{boldi2004webgraph}  }          & 978,408,098      &74,744,358,622    &  76.3 \\
{\emph{Hyperlink2014}~\cite{meusel15hyperlink}  }    & 1,724,573,718    &124,141,874,032   &  72.0 \\
{\emph{Hyperlink2012}~\cite{meusel15hyperlink}  }    & 3,563,602,789    &225,840,663,232   &  63.3 \\
\end{tabular}
\captionof{table}{\label{table:graphinfo}\small Graph inputs, number
of vertices, edges, and average degree ($\davg$).}
\label{table:sizes}
\end{table}

DRAM,reduce,0.102
DRAM,reduce-gather,1.59
NVRAM,reduce,0.255
NVRAM,reduce-gather,6.99


==> response/work_depth_bounds.tex <==
\subsection*{Common Concern 2: Work-depth Model, \SAMabbrev{} Bounds, Examples of \SAMabbrev{} Analysis}
This section is to address {\bf W2}, {\bf W3}, {\bf R1}, and {\bf R2} of Reviewer 1,
{\bf W2}, {\bf W3}, and {\bf D2} of Reviewer 2.
\answer{This revision occurs in Section 4.}
%
We thank the reviewers for their helpful comments about this topic,
which helped us improve the paper.

%W2: The selection of the algorithm cost measurement is not clear. The
%rationale for choosing the work-depth measure for the cost on PSAM
%need further details to justify why the measurement is reasonable and
%not biased.
\myparagraph{Importance of the Work-Depth Metric}
We first address Reviewer 2's question ({\bf Reviewer 2: [W2]}) about
whether the \emph{work-depth} metric is a good choice to model costs.
We choose to use work-depth since it combines simplicity, practicality, and
a strong foundation in the theoretical literature.

Algorithms designed in the work-depth model map very naturally to
practical and efficient implementations. This is true because the model
(i) does not permit forking off arbitrarily many threads in constant depth,
thereby realistically reflecting the depth of practical runs, and (ii) has
provably-efficient schedulers that can run a computation with work $W$
and depth $D$ on $p$ processors in $W/p + O(D)$ time with high
probability~\cite{blumofe1999scheduling, BBFGGMS16}.

The work-depth model has a long history of study, including a large body of
provably-efficient in-memory graph algorithms that are known in this
model, e.g., \cite{shiloach1982connectivity, karp1984mis, luby1986mis,
alon1986mis, tarjan1985efficient, Miller1992, Ramachandran89, JaJa92,
cole96minimum, pettie2000mst, miller2013parallel,
fineman2017reachability,Birn13,meyer2003delta}. Both this work and our
previous work on GBBS~\cite{dhulipala18scalable} build on this rich
theoretical literature.
%
Furthermore, the work-depth measure has been widely used in designing
provably-efficient and practically sound parallel graph algorithms,
and is a crucial tool in designing parallel algorithms. For
example, see~\cite{shun2014practical, DBLP:conf/spaa/GuSSB15,
BlellochFS16, pam, dhulipala18scalable, wang2019pardbscan,
sun2019supporting} for recent practical uses of this model in our
recent work in the context of parallel algorithms, large-scale graph
algorithms, database systems, and density-based clustering. The model
is also widely used by many other researchers to study
provably-efficient parallel algorithms, ranging from graph-algorithms,
to deterministic race-detection, cache-efficient algorithms, parallel
numerical linear-algebra, and other domains~\cite{Leiserson2010,
TangYKTGC15, Sanders2015, Kaler2016, Agrawal2018, Chowdhury2017,
Xu2018, Singer2020, Kaler2020}.

%<<<<<<< HEAD
%example, see~\cite{
%shun2014practical,
%DBLP:conf/spaa/GuSSB15,
%BlellochFS16,
%pam,
%dhulipala18scalable,
%wang2019pardbscan,
%sun2019supporting,
%akhremtsev2016fast,
%sanders2015work,
%kaler2019cilkmem,
%hasenplaugh2014ordering,
%kaler2016executing,
%singer2020scheduling,
%xu2018efficient,
%agrawal2014provably,
%workingset,
%leiserson2010bfs
%} for recent practical uses of this model in the
%context of parallel algorithms, large-scale graph algorithms, database
%systems, and density-based clustering. The model is widely used by
%other authors to study provably-efficient parallel algorithms, ranging
%from graph-algorithms, to deterministic race-detection,
%cache-efficient algorithms, parallel numerical linear-algebra, and
%other domains~\cite{Leiserson2010, TangYKTGC15, Sanders2015,
%Kaler2016, Agrawal2018, Chowdhury2017, Xu2018, Singer2020, Kaler2020}.
%=======

Lastly, we would like to emphasize the benefits of proving
good bounds on the work and depth of our algorithms in this paper.
For one, algorithms with good provable-bounds on their work and depth are more
robust to bad or adversarial inputs than algorithms based on heuristic
approaches. Another benefit of work-efficiency is that
in the parallel algorithms literature, in both theory and practice,
it has been observed that work-efficient algorithms can be significantly faster than
work-inefficient algorithms. For example, our previous
work found that our $k$-core algorithm based on work-efficient
bucketing is between 2--9x faster than a work-inefficient algorithm
that is often used in practice~\cite{dhulipala2017julienne}. Several
other recent success stories of work-efficient algorithms include
semi-sorting~\cite{DBLP:conf/spaa/GuSSB15}, parallel graph
connectivity~\cite{shun2014practical}, parallel compressed string data
structures~\cite{BlellochS11}, parallel maximal independent set,
and maximal matching~\cite{blelloch2012greedy}, to name a few.

\myparagraph{Illustrating Work-Depth Analysis}
Based on Reviewer 1's feedback (comments {\bf Reviewer 1: [W3, W1, R1,
R2]}), we made two significant changes to the paper.

The first change was to add a new subsection in Section 4,
Section 4.1.3, showing how our new semi-asymmetric graph traversal
primitive can be used to implement breadth-first search (undirected
shortest-paths).  The new section contains the full code of our BFS
implementation in \oursystem{}, a description of the algorithm, and a
complete proof of the work-depth analysis in the \SAMabbrev{}.

The second change was to make a complete re-organization of Section 4
to improve readability, and to make a significant revision of Section
4.3 where our algorithm bounds are discussed. The re-organization
included reordering the sections so that the content is introduced in
a more logical order. The revision of Section 4.3 involved separating
the descriptions of what problems we solve, and the work our codes are
based on, from the changes and improvements we make in the
\SAMabbrev{} model. We sincerely hope that these changes have improved
the readability and understandability of our approaches.






























==> semisort.tex <==
\section{Our Algorithm}
In this section, we present our semisort algorithms. Our \semieq{} is work-efficient and our \semile{} is space-efficient. \xiaojun{Check I/O and span.}
The high level idea of our algorithms is to find out the heavy keys by sampling,
partition light keys and heavy keys into their corresponding buckets,
and semisort each light bucket recursively until the base case.
In the base case, \semieq{} uses a hash table with separate chaining to partition the keys, and \semile{} uses a standard comparison sort.
Our algorithms is practical for two main reasons:
1) although keys are not heavy enough to be identified as heavy keys in a level of recursion, they can still be identified as heavy keys in the next recursive call \xiaojun{because its ratio increases}.
Heavy keys require less computation because we simply need to send all heavy keys to the destination address, and no further recursion or base case is needed;
2) we can set the base-case granularity so that all elements fit in cache, and therefore semisorting them is very fast.
\xiaojun{Credit parlay::integer\_sort.}

\subsection{Algorithm Details}
The \semieq{} and \semile{} algorithms only differ in how they solve the sequential base case,
so we only present a common algorithms framework of them.
\xiaojun{We can say we have a nice framework that also fits semisort\_integer (the hash function returns the key itself and no collision). We don't have the experiemnts though.}
The pseudocode of our framework is shown in~\cref{alg:semisort}.
Our framework consists of four steps.

\myparagraph{Sequential Base Case.}
If the input size is small enough, we can semisort them sequentially (\cref{line::basecase}).
For \semile{}, we use a standard comparison sort (e.g., quicksort).
For \semieq{}, we first build a hash table of size $n^k$. \laxman{$(1+\epsilon)n$? The hash values are $n^k$ but size is just a constant factor larger than $n$.}
Then we iterate over all keys and insert each key to the hash table with separate chaining using the hash function.
Finally, all elements are packed to the output by looping over the hash table in order.

\myparagraph{Sample Heavy Keys.}
In the parallel recursion, we start the algorithm with sampling.
We take $\beta \log n$ samples from the input (\cref{line:sample}) and count the occurrences of each key (\cref{line:count}).
Keys with at least $\log n$ occurrences are identified as heavy keys.
They are inserted to a hash table $H$ and a distinct id is assigned to each key (\cref{line:insert}).
\laxman{What about parameters used in the framework, e.g., $\threshold$ and $p$?}

\myparagraph{Count Sort.}
We can assign an id to each light key by using the $b$ lowest significant bits of its hash value.
Assume we identify $n_H$ heavy keys and use $n_L=2^b$ ids to distinguish the light keys, then all keys can be partition into $n_H+n_L$ buckets (\cref{line:bucketid}).
In this step, we first (virtually) divide the input sequence into $\sqrt{n}$ blocks, and allocate a $\counts[\cdot]$ array to indicate the number of keys in each bucket in each block.
We can count the keys of different blocks in parallel.
Within each block, the $\counts[\cdot]$ array is computed in sequential.
Then the $\offsets[\cdot]$ of each block can be computed by using a scan function,
where $\offsets[\cdot]$ denotes the starting position of each bucket of each block when the keys are partitioned.
Lastly, we partition the keys and return the $\offsets[\cdot]$ of each light bucket.

\myparagraph{Recursion.}
Now all heavy keys are contiguous but light keys can still be scattered.
We need to apply the semisort to each light bucket recursively (\cref{line:recursion}) until
1) all light buckets are empty, or
2) the input case is small enough, then it goes to the base case.




\input{algo-semisort.tex}


==> tables/graph-stat.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \small
  \begin{minipage}{\columnwidth}
  \centering
    \begin{tabular}{@{}l@{ }|rrrrrrl}
    \textbf{Dataset} & \multicolumn{1}{c}{$n$} & \multicolumn{1}{c}{$m$} & \multicolumn{1}{r}{\textbf{$n_{\mathit{dist}}$}} & \multicolumn{1}{r}{{$f_\mathit{max}$}} & \multicolumn{1}{r}{\textbf{$r_\mathit{large}$}} & \multicolumn{1}{r}{$r_\mathit{small}$} & \multicolumn{1}{c}{{source}} \\
    \midrule
    \textbf{LJ} & 4.8M  & 69M   & 4.4M  & 14K   & 0.09\% & 24.1\% & ~\cite{backstrom2006group} \\
    \textbf{SD} & 89M   & 2.0B  & 73M   & 2.3M  & 22.3\% & 12.4\% &  ~\cite{webgraph}\\
    \textbf{CW} & 978M  & 43B   & 938M  & 76M   & 17.7\% & 7.45\% &  ~\cite{webgraph}\\
    \textbf{CM} & 321M  & 1.6B  & 320M  & 17    & 0.00\% & 100\% &  ~\cite{cosmo50,wang2021geograph}\\
    \textbf{2gram} & 68M   & -     & 3.1M  & 2.2M  & 28.0\% & 11.0\% & TODO \\
    \textbf{3gram} & 224M  & -     & 47M   & 319K  & 4.43\% & 41.0\% & TODO \\
    \bottomrule
    \end{tabular}%
  \caption{\textbf{Dataset for the two applications.} In graphs, $n=$ number of vertices and $m=$ number of edges.
  $n_\mathit{dist}=$ number of distinct keys. $f_\mathit{max}=$ maximum frequency.
  $r_\mathit{large}=$ ratio of records with key appearing $\ge 500\log n$ times.
  $r_\mathit{small}=$ ratio of records with key appearing $<\log n$ times.
  %\yihan{Combine this with some other figures.}
  \yihan{add wiki citation.}
  \label{tab:graphstats}%
  }
  \end{minipage} \hfill
  %
  \begin{minipage}{0.6\columnwidth}
  \begin{tabular}{l|rr}
          & \multicolumn{1}{l}{\textbf{2-gram}} & \multicolumn{1}{l}{\textbf{3-gram}} \\
    \midrule
    \semisortequal & 0.327  & 8.46 \\
    \semisortless & 0.355  & 2.52 \\
    PLSS  & 0.387  & 2.56 \\
    ips$^4$o & 1.15  & 3.55 \\
    \end{tabular}%
    \caption{\textbf{Running time (in seconds) on semisorting n-grams. }}
  \end{minipage}

\end{table*}%


